DocMIA: Document-Level Membership Inference Attacks against DocVQA Models

Document Visual Question Answering (DocVQA) has introduced a new paradigm for end-to-end document understanding, and quickly became one of the standard benchmarks for multimodal LLMs. Automating document processing workflows, driven by DocVQA models, presents significant potential for many business sectors. However, documents tend to contain highly sensitive information, raising concerns about privacy risks associated with training such DocVQA models. One significant privacy vulnerability, exploited by the membership inference attack, is the possibility for an adversary to determine if a particular record was part of the model's training data. In this paper, we introduce two novel membership inference attacks tailored specifically to DocVQA models. These attacks are designed for two different adversarial scenarios: a white-box setting, where the attacker has full access to the model architecture and parameters, and a black-box setting, where only the model's outputs are available. Notably, our attacks assume the adversary lacks access to auxiliary datasets, which is more realistic in practice but also more challenging. Our unsupervised methods outperform existing state-of-the-art membership inference attacks across a variety of DocVQA models and datasets, demonstrating their effectiveness and highlighting the privacy risks in this domain.

==> figures/number_questions.tex <==
\begin{figure}[t]
    \centering
    \subfigure[\centering \textbf{DocVQA}]{
        \includegraphics[height=3cm,width=0.6\textwidth]{images/number_questions_DocVQA.pdf}
    }
    \subfigure[\centering \textbf{PFL-DocVQA}]{
        \includegraphics[height=3cm,width=0.36\textwidth]{images/number_questions_PFL.pdf}
    }
\caption{\textbf{Attack Accuracy vs. varying Number of Questions per Document $M$.} The horizontal axis represents bins of documents grouped by the number of questions in intervals defined by the bin edges.}
\vspace{-0.2in}
\label{fig:number_questions}
\end{figure}


==> figures/roc_whitebox_docvqa.tex <==
\begin{figure}[t]
    \centering

    \subfigure[]{
        \includegraphics[width=0.3\textwidth]{images/roc_curve_whitebox_vt5_docvqa.pdf}
        \label{fig:roc_whitebox_docvqa_vt5}
    }
    \subfigure[]{
        \includegraphics[width=0.3\textwidth]{images/roc_curve_whitebox_donut_docvqa.pdf}
        \label{fig:roc_whitebox_docvqa_donut}
    }
    \subfigure[]{
        \includegraphics[width=0.3\textwidth]{images/roc_curve_whitebox_pix2struct_docvqa.pdf}
        \label{fig:roc_whitebox_docvqa_pix2struct}
    }
    \caption{\textbf{ROC Curve DocVQA} Say sth....}
    \label{fig:roc_whitebox_docvqa}
\end{figure}



==> figures/roc_whitebox_pfl.tex <==
\begin{figure}[t]
    \centering

    \subfigure[]{
        \includegraphics[width=0.32\textwidth]{images/roc_curve_whitebox_vt5_docvqa.pdf}
        \label{fig:roc_whitebox_pfl_vt5}
    }
    \subfigure[]{
        \includegraphics[width=0.32\textwidth]{images/roc_curve_whitebox_donut_docvqa.pdf}
        \label{fig:roc_whitebox_pfl_donut}
    }
    \caption{\textbf{ROC Curve PFL-DocVQA} Say sth....}
    \label{fig:roc_whitebox_pfl}
\end{figure}



==> tables/baseline_updated_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
\begin{adjustbox}{width=\textwidth}
\small
\begin{tabular}{clcccccccccccccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{$\textsc{Score-TA}$} & \multicolumn{2}{c}{$\textsc{Score-UA}$} & \multicolumn{2}{c}{$\textsc{Score-UA}_{\text{all}}$} & \multicolumn{2}{c}{$\textsc{Loss-TA}$} & \multicolumn{2}{c}{$\textsc{Gradient-UA}$} & \multicolumn{2}{c}{$\textsc{ScoreLoss-UA}_{\text{all}}$} & \multicolumn{2}{c}{$\text{Min-K\%}^{\dagger}$} & \multicolumn{2}{c}{$\text{Min-K\%++}^{\dagger}$}\\
\cmidrule(l){3-4}
\cmidrule(l){5-6}
\cmidrule(l){7-8}
\cmidrule(l){9-10}
\cmidrule(l){11-12}
\cmidrule(l){13-14}
\cmidrule(l){15-16}
\cmidrule(l){17-18}
& & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 \\
\midrule 
\multirow{2}{*}{\rotatebox[origin=c]{90}{PFL}}& {VT5} & \cellcolor[HTML]{C0C0C0}{$\textbf{62.33}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{64.13}$} & \cellcolor[HTML]{C0C0C0}{$61.00_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$68.80_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$60.67_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$60.67_{0.0}$} & $57.83$ & $62.81$ & $60.67_{0.0}$ & $60.67_{0.0}$ & $60.67_{0.0}$ & $60.67_{0.0}$ & 57.17 & 64.84 & \textbf{61.33} & \textbf{72.16}\\

& {Donut} & \cellcolor[HTML]{C0C0C0}{$\textbf{73.33}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{75.14}$} & \cellcolor[HTML]{C0C0C0}{$68.33_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$75.77_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$71.17_{0.67}$} & \cellcolor[HTML]{C0C0C0}{$71.33_{3.32}$} & $\textbf{73.67}$ & $\textbf{78.99}$ & $70.67_{0.0}$ & $69.55_{0.0}$ & $70.83_{0.0}$ & $69.67_{0.0}$ & 36.5 & 32.09 & 50.5 & 60.35\\
\midrule

\multirow{3}{*}{\rotatebox[origin=c]{90}{DVQA}} & {VT5} & \cellcolor[HTML]{C0C0C0}{$\textbf{75.67}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{75.75}$} & \cellcolor[HTML]{C0C0C0}{$72.17_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$76.18_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$75.17_{0.0}$} & \cellcolor[HTML]{C0C0C0}{$75.13_{0.0}$} & $73.67$ & $77.99$ & $71.17_{0.0}$ & $67.54_{0.0}$ & $\textbf{75.50}_{\textbf{0.0}}$ & $\textbf{76.02}_{\textbf{0.0}}$ & 71.0 & 76.16 & 66.67 & 74.56 
\\

& {Donut} & \cellcolor[HTML]{C0C0C0}{$79.67$} & \cellcolor[HTML]{C0C0C0}{$79.53$} & \cellcolor[HTML]{C0C0C0}{$75.97_{0.07}$} & \cellcolor[HTML]{C0C0C0}{$79.57_{0.07}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{80.50}_{\textbf{0.0}}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{81.10}_{\textbf{0.0}}$} & $51.83$ & $53.46$ & $77.17_{0.0}$ & $75.92_{0.0}$ & $\textbf{80.50}_{\textbf{0.0}}$ & $\textbf{81.10}_{\textbf{0.0}}$ & 47.0 & 48.38 & 53.33 & 59.89
\\

& {Pix2Struct-B} & \cellcolor[HTML]{C0C0C0}{$67.33$} & \cellcolor[HTML]{C0C0C0}{$67.97$} & \cellcolor[HTML]{C0C0C0}{$\textbf{68.17}_{\textbf{0.0}}$} & \cellcolor[HTML]{C0C0C0}{$\textbf{71.36}_{\textbf{0.0}}$} & \cellcolor[HTML]{C0C0C0}{$69.13_{0.07}$} & \cellcolor[HTML]{C0C0C0}{$67.67_{0.09}$} & $59.33$ & $64.63$ & $66.0_{0.0}$ & $68.32_{0.0}$ & $\textbf{69.00}_{\textbf{0.0}}$ & $\textbf{67.48}_{\textbf{0.0}}$ & 68.0 & 72.8 & 54.50 & 66.99
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\caption{\textbf{Results from Baseline Attacks.}. \textcolor{gray}{\textbf{Gray}} color indicate attacks conducted in the black-box setting. $\dagger$ indicates methods requiring grey-box access. Results are reported based on five random seeds for \textsc{KMeans}, if any. The methods with the best \textit{average} performance across the two metrics are highlighted in \textbf{bold}.}
\vspace{-0.2in}
\label{tab:baseline_updated_results}
\end{table}


==> tables/blackbox_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
\begin{adjustbox}{width=0.8\textwidth}
\small
\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{c}{Proxy Model} & \multicolumn{6}{c}{VT5}\\

\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Black-box}}} & \multicolumn{2}{c}{FL} & \multicolumn{2}{c}{FLLoRA} & \multicolumn{2}{c}{IG}\\
%\cmidrule{3-8}
\cmidrule(l){3-4}
\cmidrule(l){5-6}
\cmidrule(l){7-8}
&                                 & ACC & F1 & ACC & F1 & ACC & F1\\
\midrule 
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{PFL}}}& \textbf{VT5} & $63.33_{0.0}\textcolor{red}{(+2.33)}$ & $69.51_{0.03}\textcolor{red}{(+0.71)}$ & $63.33_{0.0}\textcolor{red}{(+2.33)}$ & $69.01_{0.0}\textcolor{red}{(+0.21)}$ & $62.00_{0.16}\textcolor{red}{(+1)}$ & $69.35_{0.2}\textcolor{red}{(+0.55)}$\\

& \textbf{Donut} & $70.83_{0.0}\textcolor[HTML]{0b5394}{(-0.34)}$ & $76.64_{0.0}\textcolor{red}{(+0.87)}$ & $70.83_{0.0}\textcolor[HTML]{0b5394}{(-0.34)}$ & $76.70_{0.0}\textcolor{red}{(+0.93)}$ & $70.67_{0.0}\textcolor[HTML]{0b5394}{(-0.5)}$ & $76.72_{0.0}\textcolor{red}{(+0.95)}$\\
\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{DVQA}}}& \textbf{VT5} & $74.33_{0.01}\textcolor[HTML]{0b5394}{(-0.84)}$ & $75.08_{0.0}\textcolor[HTML]{0b5394}{(-1.1)}$ & $74.33_{0.0}\textcolor[HTML]{0b5394}{(-0.84)}$ & $74.67_{0.0}\textcolor[HTML]{0b5394}{(-1.51)}$ & $73.83_{0.08}\textcolor[HTML]{0b5394}{(-1.34)}$ & $75.81_{0.0}\textcolor[HTML]{0b5394}{(-0.37)}$\\

& \textbf{Donut} & $81.67_{0.0}\textcolor{red}{(+1.17)}$ & $82.54_{0.0}\textcolor{red}{(+1.44)}$ & $81.17_{0.0}\textcolor{red}{(+0.67})$ & $82.09_{0.0}\textcolor{red}{(+0.99)}$ & $80.17_{0.0}\textcolor[HTML]{0b5394}{(-0.33)}$ & $81.89_{0.0}\textcolor{red}{(+0.79)}$\\

& \textbf{Pix2Struct-B} & $70.17_{0.0}\textcolor{red}{(+1.04)}$ & $69.71_{0.0}\textcolor[HTML]{0b5394}{(-1.65})$ & $70.27_{0.23}\textcolor{red}{(+1.14)}$ & $70.85_{0.07}\textcolor[HTML]{0b5394}{(-0.51)}$ & $71.17_{0.0}\textcolor{red}{(+2.04)}$ & $72.14_{0.0}\textcolor{red}{(+0.78)}$\\

\cmidrule{2-8}
& \textbf{Pix2Struct-L} & $71.67_{0.01}\textcolor{red}{(+0.84)}$ & $72.13_{0.0}\textcolor{red}{(+1.30)}$ & $70.17_{0.0}\textcolor[HTML]{0b5394}{(-0.66)}$ & $71.27_{0.0}\textcolor{red}{(+0.44)}$ & $71.00_{0.05}\textcolor{red}{(+0.17)}$ & $73.15_{0.0}\textcolor{red}{(+2.32)}$\\

\midrule
\multicolumn{2}{c}{Proxy Model} & \multicolumn{6}{c}{Donut}\\ 

\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{PFL}}}& \textbf{VT5} & $61.73_{0.08}\textcolor{red}{(+0.73)}$ & $64.04_{0.10}\textcolor[HTML]{0b5394}{(-4.76)}$ & $61.67_{0.08}\textcolor{red}{(+0.67)}$ & $63.49_{0.0}\textcolor[HTML]{0b5394}{(-5.31)}$ & $55.17_{0.17}\textcolor[HTML]{0b5394}{(-5.83)}$ & $57.37_{0.3}\textcolor[HTML]{0b5394}{(-11.43)}$\\

& \textbf{Donut} & $72.17_{0.0}\textcolor{red}{(+2.33)}$ & $76.24_{0.0}\textcolor[HTML]{0b5394}{(-0.19)}$ & $72.67_{0.0}\textcolor{red}{(+1.5)}$ & $77.47_{0.0}\textcolor{red}{(+1.7)}$ & $74.50_{0.0}\textcolor{red}{(+3.33)}$ & $76.43_{0.0}\textcolor{red}{(+0.66)}$\\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{DVQA}}}& \textbf{VT5} & $73.50_{0.0}\textcolor[HTML]{0b5394}{(-4.34)}$ & $75.58_{0.0}\textcolor[HTML]{0b5394}{(-4.36)}$ & $74.17_{0.0}\textcolor[HTML]{0b5394}{(-1)}$ & $76.04_{0.0}\textcolor[HTML]{0b5394}{(-0.14)}$ & $74.0_{0.0}\textcolor[HTML]{0b5394}{(-1.17)}$ & $75.93_{0.01}\textcolor[HTML]{0b5394}{(-0.25)}$\\

& \textbf{Donut} & $79.50_{0.0}\textcolor[HTML]{0b5394}{(-1)}$ & $81.50_{0.0}\textcolor{red}{(+0.4)}$ & $80.0_{0.0}\textcolor[HTML]{0b5394}{(-0.5)}$ & $81.82_{0.0}\textcolor{red}{(+0.72)}$ & $80.27_{0.0}\textcolor[HTML]{0b5394}{(-0.23)}$ & $81.96_{0.0}\textcolor{red}{(+0.86)}$\\

& \textbf{Pix2Struct-B} & $70.83_{0.0}\textcolor{red}{(+3.04)}$ & $71.82_{0.0}\textcolor{red}{(+4.88)}$ & $70.83_{0.06}\textcolor{red}{(+1.70)}$ & $71.73_{0.14}\textcolor{red}{(+0.37)}$ & $71.0_{0.01}\textcolor{red}{(+1.87)}$ & $71.94_{0.0}\textcolor{red}{(+0.58)}$\\

\cmidrule{2-8}
& \textbf{Pix2Struct-L} & $70.83_{0.0}{(0)}$ & $72.95_{0.0}\textcolor{red}{(+2.12)}$ & $71.0_{0.0}\textcolor{red}{(+0.17)}$ & $72.98_{0.0}\textcolor{red}{(+2.15)}$ & $71.0_{0.03}\textcolor{red}{(+0.17)}$ & $72.81_{0.01}\textcolor{red}{(+1.98)}$\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}

\caption{\textbf{Black-Box Setting: Main Results of Black-Box \atk using Donut and VT5 as proxy models}. The checkpoints for the \textbf{black-box models} are trained on the respective datasets. Values in parentheses indicate the improvement (\textcolor{red}{positive}/\textcolor[HTML]{0b5394}{negative}) compared to the \textit{best} number from $\textsc{Score-UA}$-based baselines. Results are reported over five random seeds.}
\vspace{-0.2in}
\label{tab:blackbox_results}
\end{table}

==> tables/blackbox_results_donut.tex <==
\begin{table}[t]
\vskip 0.15in
\begin{center}
\begin{small}
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Black-box}}} & \multicolumn{2}{c}{FL} & \multicolumn{2}{c}{FLLoRA} & \multicolumn{2}{c}{IG}\\
\cmidrule{3-8}
&                                 & ACC & F1 & ACC & F1 & ACC & F1\\
\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{PFL}}& \textbf{VT5} & $61.73_{0.08}\textcolor{red}{(+0.73)}$ & $64.04_{0.10}\textcolor{blue}{(-4.76)}$ & $61.67_{0.08}\textcolor{red}{(+0.67)}$ & $63.49_{0.0}\textcolor{blue}{(-5.31)}$ & $55.17_{0.17}\textcolor{blue}{(-5.83)}$ & $57.37_{0.3}\textcolor{blue}{(-11.43)}$\\

& \textbf{Donut} & $72.17_{0.0}\textcolor{red}{(+2.33)}$ & $76.24_{0.0}\textcolor{blue}{(-0.19)}$ & $72.67_{0.0}\textcolor{red}{(+1.5)}$ & $77.47_{0.0}\textcolor{red}{(+1.7)}$ & $74.50_{0.0}\textcolor{red}{(+3.33)}$ & $76.43_{0.0}\textcolor{red}{(+0.66)}$\\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{DVQA}}& \textbf{VT5} & $73.50_{0.0}\textcolor{blue}{(-4.34)}$ & $75.58_{0.0}\textcolor{blue}{(-4.36)}$ & $74.17_{0.0}\textcolor{blue}{(-1)}$ & $76.04_{0.0}\textcolor{blue}{(-0.14)}$ & $74.0_{0.0}\textcolor{blue}{(-1.17)}$ & $75.93_{0.01}\textcolor{blue}{(-0.25)}$\\

& \textbf{Donut} & $79.50_{0.0}\textcolor{blue}{(-1)}$ & $81.50_{0.0}\textcolor{red}{(+0.4)}$ & $80.0_{0.0}\textcolor{blue}{(-0.5)}$ & $81.82_{0.0}\textcolor{red}{(+0.72)}$ & $80.27_{0.0}\textcolor{blue}{(-0.23)}$ & $81.96_{0.0}\textcolor{red}{(+0.86)}$\\

& \textbf{Pix2struct-B} & $70.83_{0.0}\textcolor{red}{(+3.04)}$ & $71.82_{0.0}\textcolor{red}{(+4.88)}$ & $70.83_{0.06}\textcolor{red}{(+1.70)}$ & $71.73_{0.14}\textcolor{red}{(+0.37)}$ & $71.0_{0.01}\textcolor{red}{(+1.87)}$ & $71.94_{0.0}\textcolor{red}{(+0.58)}$\\

\cmidrule{2-8}
& \textbf{Pix2struct-L} & $70.83_{0.0}{(0)}$ & $72.95_{0.0}\textcolor{red}{(+2.12)}$ & $71.0_{0.0}\textcolor{red}{(+0.17)}$ & $72.98_{0.0}\textcolor{red}{(+2.15)}$ & $71.0_{0.03}\textcolor{red}{(+0.17)}$ & $72.81_{0.01}\textcolor{red}{(+1.98)}$\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\caption{\textbf{Black-Box: Results using Donut as the proxy model}. The checkpoints for the \textbf{black-box models} are trained on the respective datasets. Results are reported over 5 random seeds.}
\label{tab:blackbox_results_donut}
\end{table}

==> tables/blackbox_results_vt5.tex <==
\begin{table}[t]
\vskip 0.15in
\begin{center}
\begin{small}
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Black-box}}} & \multicolumn{2}{c}{FL} & \multicolumn{2}{c}{FLLoRA} & \multicolumn{2}{c}{IG}\\
\cmidrule{3-8}
&                                 & ACC & F1 & ACC & F1 & ACC & F1 \\
\midrule 
\multirow{2}{*}{\rotatebox[origin=c]{90}{PFL}}& \textbf{VT5} & $63.33_{0.0}\textcolor{red}{(+2.33)}$ & $69.51_{0.03}\textcolor{red}{(+0.71)}$ & $63.33_{0.0}\textcolor{red}{(+2.33)}$ & $69.01_{0.0}\textcolor{red}{(+0.21)}$ & $62.0_{0.16}\textcolor{red}{(+1)}$ & $69.35_{0.2}\textcolor{red}{(+0.55)}$\\

& \textbf{Donut} & $70.83_{0.0}\textcolor{blue}{(-0.34)}$ & $76.64_{0.0}\textcolor{red}{(+0.87)}$ & $70.83_{0.0}\textcolor{blue}{(-0.34)}$ & $76.70_{0.0}\textcolor{red}{(+0.93)}$ & $70.67_{0.0}\textcolor{blue}{(-0.5)}$ & $76.72_{0.0}\textcolor{red}{(+0.95)}$\\
\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{DVQA}}& \textbf{VT5} & $74.33_{0.01}\textcolor{blue}{(-0.84)}$ & $75.08_{0.0}\textcolor{blue}{(-1.1)}$ & $74.33_{0.0}\textcolor{blue}{(-0.84)}$ & $74.67_{0.0}\textcolor{blue}{(-1.51)}$ & $73.83_{0.08}\textcolor{blue}{(-1.34)}$ & $75.81_{0.0}\textcolor{blue}{(-0.37)}$\\

& \textbf{Donut} & $81.67_{0.0}\textcolor{red}{(+1.17)}$ & $82.54_{0.0}\textcolor{red}{(+1.44)}$ & $81.17_{0.0}\textcolor{red}{(+0.67})$ & $82.09_{0.0}\textcolor{red}{(+0.99)}$ & $80.17_{0.0}\textcolor{blue}{(-0.33)}$ & $81.89_{0.0}\textcolor{red}{(+0.79)}$\\

& \textbf{Pix2struct-B} & $70.17_{0.0}\textcolor{red}{(+1.04)}$ & $69.71_{0.0}\textcolor{blue}{(-1.65})$ & $70.27_{0.23}\textcolor{red}{(+1.14)}$ & $70.85_{0.07}\textcolor{blue}{(-0.51)}$ & $71.17_{0.0}\textcolor{red}{(+2.04)}$ & $72.14_{0.0}\textcolor{red}{(+0.78)}$\\

\cmidrule{2-8}
& \textbf{Pix2struct-L} & $71.67_{0.01}\textcolor{red}{(+0.84)}$ & $72.13_{0.0}\textcolor{red}{(+1.30)}$ & $70.17_{0.0}\textcolor{blue}{(-0.66)}$ & $71.27_{0.0}\textcolor{red}{(+0.44)}$ & $71.0_{0.05}\textcolor{red}{(+0.17)}$ & $73.15_{0.0}\textcolor{red}{(+2.32)}$\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\caption{\textbf{Black-Box: Results using VT5 as the proxy model}. The checkpoints for the \textbf{black-box models} are trained on the respective datasets. Results are reported over 5 random seeds.}
\label{tab:blackbox_results_vt5}
\end{table}


==> tables/tpr_fpr_whitebox_docvqa.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{VT5} & \multicolumn{3}{c}{Donut} & \multicolumn{3}{c}{Pix2Struct-B} \\
\cmidrule(l){2-4}
\cmidrule(l){5-7}
\cmidrule(l){8-10}
 & TPR1\%FPR & TPR3\%FPR & TPR5\%FPR & TPR1\%FPR & TPR3\%FPR & TPR5\%FPR & TPR1\%FPR & TPR3\%FPR & TPR5\%FPR \\
\midrule
$\textsc{Score-TA}$ & 2.67 & 17.33 & 24.33 & 1.00 & 3.67 & 9.67 & 1.00 & 4.67 & 11.33 \\
$\textsc{Score-UA}$ & 3.00 & 9.33 & 13.33 & 3.33 & 7.00 & 12.00 & 3.33 & 9.00 & 11.00 \\
$\textsc{Score-UA}_{\text{all}}$ & 2.67 & 17.33 & 24.33 & 1.00 & 3.67 & 9.67 & 1.00 & 4.67 & 11.33 \\
\midrule
$\textsc{Loss-TA}$ & 4.67 & \textbf{19.33} & \textbf{25.33} & 0.67 & 7.67 & 9.33 & 2.33 & 5.33 & 9.33 \\
$\textsc{Gradient-UA}$ & 4.00 & 15.33 & 21.33 & \textbf{3.67} & 6.00 & 12.67 & 1.00 & 5.00 & 8.00 \\
$\textsc{ScoreLoss-UA}_{\text{all}}$ & 1.33 & 4.67 & 11.33 & 2.67 & 8.67 & 11.67 & 2.00 & 6.67 & 10.00 \\
\midrule
FL & 3.67 & 8.00 & 16.00 & 3.33 & \textbf{10.67} & \textbf{15.67} & \textbf{6.00} & \textbf{11.00} & 15.00 \\
FLLoRA & \textbf{5.33} & 18.33 & 24.67 & 2.67 & 5.33 & 8.00 & 3.67 & 6.33 & 7.33 \\
IG & 2.00 & 8.67 & 15.00 & 1.33 & 8.67 & 15.00 & 3.00 & 10.33 & \textbf{15.67} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\caption{\khanh{Updated content: \textbf{TPR at fixed FPR on DocVQA}. Comparison across all methods, with the best-performing method for each metric highlighted in \textbf{bold}.}}
\label{tab:tpr@fpr_docvqa}
\end{table}


==> tables/tpr_fpr_whitebox_pfl.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{VT5} & \multicolumn{3}{c}{Donut} \\
\cmidrule(l){2-4}
\cmidrule(l){5-7}
 & TPR1\%FPR & TPR3\%FPR & TPR5\%FPR & TPR1\%FPR & TPR3\%FPR & TPR5\%FPR \\
\midrule
$\textsc{Score-TA}$ & 1.33 & 6.00 & 12.00 & \textbf{2.67} & 6.33 & 12.33\\
$\textsc{Score-UA}$ & 2.00 & 4.00 & 8.33 & 1.33 & 2.67 & 9.67 \\
$\textsc{Score-UA}_{\text{all}}$ & 1.33 & 7.00 & 12.00 & 2.67 & 6.33 & 12.33 \\
\midrule
$\textsc{Loss-TA}$ & 0.67 & 3.00 & 6.00 & 1.67 & \textbf{13.33} & 16.67 \\
$\textsc{Gradient-UA}$ & 0.33 & 3.00 & 5.33 & 1.00 & 5.33 & 13.67 \\
$\textsc{ScoreLoss-UA}_{\text{all}}$ & 0.33 & 4.00 & 6.00 & 2.33 & 6.67 & \textbf{17.67} \\
\midrule
FL & \textbf{3.67} & \textbf{8.67} & \textbf{14.33} & 1.33 & 4.67 & 9.00 \\
FLLoRA & 1.33 & 3.33 & 7.00 & 2.00 & 6.00 & 9.67 \\
IG & 1.00 & 2.33 & 5.00 & 2.33 & 9.67 & 14.00 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\caption{\khanh{Updated content: \textbf{TPR at fixed FPR on PFL-DocVQA}. Comparison across all methods, with the best-performing method for each metric highlighted in \textbf{bold}.}}
\label{tab:tpr@fpr_pfl}
\end{table}

